Creep Tide Model for the 3-Body Problem. The rotational evolution of a circumbinary planet

We present a tidal model for treating the rotational evolution in the general three-body problem with arbitrary viscosities, in which all the masses are considered to be extended and all the tidal interactions between pairs are taken into account. Based on the creep tide theory, we present the set of differential equations that describes the rotational evolution of each body, in a formalism that is easily extensible to the N tidally-interacting body problem. We apply our model to the case of a circumbinary planet and use a Kepler-38 like binary system as a working example. We find that, in this low planetary eccentricity case, the most likely final stationary rotation state is the 1:1 spin-orbit resonance, considering an arbitrary planetary viscosity inside the estimated range for the solar system planets. We derive analytical expressions for the mean rotational stationary state, based on high-order power series of the semimajor axes ratio a1 /a2 and low-order expansions of the eccentricities. These are found to reproduce very accurately the mean behaviour of the low-eccentric numerical integrations for arbitrary planetary relaxation factors, and up to a1/a2 \sim 0.4. Our analytical model is used to predict the stationary rotation of the Kepler circumbinary planets and find that most of them are probably rotating in a sub-synchronous state, although the synchrony shift is much less important than the one estimated in Zoppetti et al. (2019, 2020). We present a comparison of our results with those obtained with the Constant Time Lag and find that, unlike what we assumed in our previous works, the cross torques have a non-negligible net secular contribution, and must be taken into account when computing the tides over each body in an N-extended-body system from an arbitrary reference frame. These torques are naturally taken into account in the creep theory.

==> articulo.tex <==
\begin{document} 


   \title{Creep Tide Model for the 3-Body Problem}

   \subtitle{I. The rotational evolution of the external body} 

   \author{G. Wuchterl
          \inst{1}
          \and
          C. Ptolemy\inst{2}\fnmsep%\thanks{mail}
          }

   \institute{Institute for Astronomy (IfA), University of Vienna,
              T\"urkenschanzstrasse 17, A-1180 Vienna\\
              \email{wuchterl@amok.ast.univie.ac.at}
         \and
             University of Alexandria, Department of Geography, ...\\
             \email{c.ptolemy@hipparch.uheaven.space}
             %\thanks{The university of heaven temporarily does not
             %        accept e-mails}
             }

   \date{Received September 15, 1996; accepted March 16, 1997}

% \abstract{}{}{}{}{} 
% 5 {} token are mandatory
 
  \abstract
  % context heading (optional)
  % {} leave it empty if necessary  
   {}
  % aims heading (mandatory)
   {}
  % methods heading (mandatory)
   {}
  % results heading (mandatory)
   {}
  % conclusions heading (optional), leave it empty if necessary 
   {}

   \keywords{ planet-star interactions -- planets and satellites: dynamical evolution and stability -- methods: analytical      }

   \maketitle
%
%-------------------------------------------------------------------

\section{Introduction}

We study the motion of three bodies with masses $m_0$, $m_1$ and $m_2$ under the effects of their mutual gravitational interactions and tides. We will employ the creep tidal model (Ferraz-Mello 2013, 2015) in its closed form (Folonier \& Ferraz-Mello 2018), extended to the case of three interacting masses. Thus, the tidal bulge raised on each $m_i$ will be the sum of the deformations generated by the other two masses.
   
%--------------------------------------------------------------------
\section{The tidal model}

We consider the extended three-body problem with masses $m_i$, $m_j$ and $m_k$ with respective radius $\mathcal{R}_i$,$\mathcal{R}_j$ and $\mathcal{R}_k$. In addition, we assume that the orbital motion of the bodies lies in the same plane while the spin vectors are perpendicular to it.

From an arbitrary inertial frame, let ${\bf R}_i$, ${\bf R}_j$ and ${\bf R}_k$ be the respective position vectors of $m_i$, $m_j$ and $m_k$. The relative position of $m_j$ to $m_i$ is denoted by ${\bf \Delta}_{ji}={\bf R}_j - {\bf R}_i$ while the angle subtended between the position of $m_j$ and the reference axis, as seen from $m_i$ is denoted by $\varphi_{ji}$ (see Figure \ref{3c}).
\begin{figure}[t!]
\centering
\includegraphics*[width=0.7\columnwidth]{fig001.jpg}
%\vspace*{-1.5cm}
\caption{The three-body problem from an inertial frame and from a $m_i$-relative frame }
\label{3c}
\end{figure}

\subsection{Equilibrium figure}

\begin{figure*}[h!]
\centering
\includegraphics*[width=0.9\textwidth]{fig002.jpg}
%\vspace*{-1.5cm}
\caption{{\it{Left: Equilibrium ellipsoid in the 3BP}}. Dashed-empty ellipsoids correspond to
the static tidal deformations generated by each of the perturbing masses, while the resulting equilibrium figure of $m_i$ (Equation (\ref{eq:ronew}) is shown by a filled gray ellipsoid. The unit vector 
${\hat {\bf r}}^{(eq)}_i$ indicates the orientation of the equivalent equilibrium bulge. {\it{Right: Real ellipsoid in the 3BP. The dark grey filled ellipsoid represents the "real" figure induced on $m_i$ when we take into account the internal viscosity. Note that it is displaced by an angle $\delta_i$ respect to the equilibrium figure and also has different tidal and rotational flattenings.}} }
\label{fig1}
\end{figure*}

As a consequence of the gravitational interaction on extended bodies, each mass undergo a deformation. The complete deformation induced on each mass $m_i$ will be the superposition of the tidal deformation due to the two companions $m_j$ and $m_k$, plus the rotational flattening due to its own spin. In this work, we consider that the deformation on each body due to these effects is small enough that a model developed up to the first order of flattening (as the one we will develop in this work) represents an accurate description of the problem.  

If we consider the static tide on $m_i$ (i.e. $m_i$ is a fluid that instantly responds to any stress), an arbitrary point on its surface with co-latitude angle $\theta$ and longitude angle $\varphi$, will be located at a distance $\rho_i$ from the gravity center, which can be expressed as (\cite{Tisserand1891,Folonier2015})
\begin{equation}
\begin{split}
\rho_{i}({\theta},{\varphi}) &=  \mathcal{R}_i \bigg[ 1 + \epsilon^{z}_i \biggl( \frac{1}{3} - \cos^2{ \theta} \biggr) \\
&+ \frac{1}{2} \sin^2{\theta}  \biggl( \epsilon^{\rho}_{ij} \cos{(2{
\varphi} - 2 \varphi_{ji})} + \epsilon^{\rho}_{ik} \cos{(2{ \varphi} - 2 \varphi_{ki})} \biggr)\bigg] 
\end{split}
\label{eq:roi}
\end{equation}
where $\mathcal{R}_i$ is the mean radius of the body $m_i$ and we have chosen the same definitions for the flattening as in \cite{Folonier2018}, given by
\begin{eqnarray}
\label{eij}
\epsilon_{ij}^{\rho} &=& \frac{15 m_j \mathcal{R}_i^3}{4 m_i \Delta^3_{ji}}  \\
\epsilon_{ij}^{z} &=& \epsilon_i^M + \frac{\epsilon_{ij}^{\rho}}{2}  \ \ \ \ \text{with} \ \ \ \ \epsilon_i^M = \frac{5 \mathcal{R}_i^3 \Omega_i^2}{4 m_i \mathcal{G}}  
\end{eqnarray}

Then, we propose that the equilibrium figure expressed in Equation (\ref{eq:roi}) corresponds to a flatted ellipsoid with equivalent equilibrium flattenings $\epsilon_i^{\rho}$ and $\epsilon_i^{z}$ and equivalent equilibrium orientation defined by the unit vector ${\hat {\bf r}}^{eq}_i = (\cos{\varphi^{eq}_i},\sin{\varphi^{eq}_i})$ (see Figure \ref{fig1}). The surface equation of this equivalent equilibrium figure can then be written as 
\begin{equation}
\begin{split}
\rho_{i}({\theta},{\varphi}) 
&= \mathcal{R}_i \bigg[1 + \epsilon^{z}_i ( \frac{1}{3} - \cos^2{\theta} ) + \frac{\epsilon^{\rho}_{i}}{2}  \sin^2{\theta} \cos{(2\varphi-2\varphi_i^{eq})}  \biggr]
\end{split}
\label{eq:ronew}
\end{equation}

It is possibly to obtain the equivalent flattenings and orientation in terms of the two-body interacting ellipsoids by equating Equation (\ref{eq:ronew}) and Equation (\ref{eq:roi}). This results in  
\begin{eqnarray}
\epsilon_i^{z} &=& \frac{1}{2}\bigg( \epsilon_{ij}^{\rho} + \epsilon_{ik}^{\rho}  \bigg) + \epsilon_{i}^{M} \nonumber \\
{(\epsilon_i^{\rho})}^2 &=& {(\epsilon_{ij}^{\rho})}^2 + {(\epsilon_{ik}^{\rho})}^2 + 2 \epsilon_{ij}^{\rho} \epsilon_{ik}^{\rho} \cos{(2\varphi_{ji}-2\varphi_{ki})}  \\
\tan{(2 \varphi_i^{eq})} &=& \frac{ \epsilon_{ij}^{\rho}\sin{(2\varphi_{ji})}+\epsilon_{ik}^{\rho}\sin{(2\varphi_{ki})} }{\epsilon_{ij}^{\rho}\cos{(2\varphi_{ji})}+\epsilon_{ik}^{\rho}\cos{(2\varphi_{ki})}} \nonumber
\label{formaeq}
\end{eqnarray}

\subsection{Creep equations}

Now, we assume that each body has a certain viscosity that does not allow it to attain the 
equilibrium figure instantaneously. For this reason, we model the real shape $\zeta_{i}({ 
\theta},{\varphi})$ of $m_i$ by a flat ellipsoid slightly different from the equilibrium one, characterized by the tidal flattening ${\mathcal E}_i^{\rho}$ and rotational flattening ${\mathcal 
E}_i^{z}$. The orientation of the real figure is angular displaced by a lag $\delta_i$ respect to the equilibrium orientation
and therefore the orientation unit vector is 
${\hat {\bf r}}^{(b)}_i = 
(\cos{(\varphi^{(eq)}_i+\delta_i)}, \sin{(\varphi^{(eq)}_i+\delta_i)})$ (see right panel in Figure \ref{fig1}).
The surface equation of the real flat ellipsoid is then given by
\begin{equation}
\zeta_i(\theta,\varphi) =\mathcal{R}_i 
\bigg[ 1 +  {\mathcal E}_i^{z} ( \frac{1}{3} - \cos^2{\theta} )+\frac{{\mathcal E}_i^{\rho}}{2}  \sin^2{\theta} \cos{(2 (\varphi_{i}^{eq} +\delta_i)-2 \varphi )}  \bigg].
\label{eq9}
\end{equation}
Contrary to Darwin-based tidal models, we  assume that the set $({\mathcal E}_i^{\rho}, {\mathcal E}_i^{z},\delta_i)$ are {\it{a-priori}} unknown quantities, 
and their values at each instant of time is obtained by solving the creep equation:
\begin{eqnarray}
\label{eq:creep}
\dot{\zeta}_i + \gamma_i \zeta_i = \gamma_i \rho_i ,
\end{eqnarray}
where $\gamma_i$ is the so-called relaxation factor 
of $m_i$ (\cite{FerrazMello2013}) and will be assumed as constant in this work.

A set of three differential equations for the shape and orientation of the real figure of $m_i$ can be obtained by differentiating Equation (\ref{eq9}) with respect to time, introducing its expression plus Equations (\ref{eq:ronew}) and (\ref{eq9}) into Equation (\ref{eq:creep}) and identifying terms of equal dependence with $(\theta,\varphi)$ (see \cite{Folonier2018}). Particularly, it is convenient to express the tidal flattening and orientation in terms of regular variables as \citep{Gomes2019} 
\begin{eqnarray}
\label{eq:forma}
\dot{X_i} &=& -\gamma_i X_i -2 Y_i (\Omega_i-\dot{\varphi_i}^{eq})+\gamma_i \epsilon_i^{\rho} \nonumber \\
\dot{Y_i} &=& -\gamma_i Y_i +2 X_i (\Omega_i-\dot{\varphi_i}^{eq})\\
\dot{{\mathcal E}_i^{z}} &=& \gamma_i ({\epsilon_i}^{z} - {{\mathcal E}_i}^{z}) \nonumber
\end{eqnarray}
where the regular variables are defined as 
\begin{eqnarray}
X_i = {\mathcal E}_i^{\rho} \cos(2\delta_i) \ \ \ \ &;& \ \ \ \ Y_i = {\mathcal E}_i^{\rho} \sin(2\delta_i) 
\end{eqnarray}

Comparing Equation (\ref{eq:forma}) with the shape and orientation evolution equations in the 2BP equation (\cite{Folonier2018,Gomes2019}, we note that in the 3BP the creep equations maintain the same form which make the formalism applicable to any N-body problem, 
being the complexity in the calculation of the corresponding equilibrium figure. CULO

\subsection{Tidal forces and torques}

At any instant of time, CULO it is possible to calculate the real shape and orientation of any body $m_i$, by solving the differential equation system $(\ref{eq:forma})$. Knowing the real flattenings and orientation of any ellipsoid, it is then possible to calculate the tidal forces and torques between the bodies.

The tidal potential due to the deformation of $m_i$ induced on $m_j$ can be calculated as (for example, \cite{Murray1999})
\begin{eqnarray}
\begin{split}
U_{ji}({\bf{\Delta}}_{ji}) &= -\frac{{\cal G} (B_i-A_i)}{2\Delta_{ji}^3}\Big(3  ({{\bf{\hat{\Delta}}}_{ji}\cdot{\bf{\hat{r}}}_i^{b}})^2 - 1 \Big)-\frac{{\cal G} (C_i-B_i)}{2\Delta_{ji}^3},
\end{split}
\label{eq13}
\end{eqnarray}

\begin{eqnarray}
\begin{split}
U_{ji}({\bf{\Delta}}_{ji}) &= -\frac{{\cal G} \mathcal{C}_i {\mathcal E}^{\rho}_i}{2\Delta_{ji}^3}\Big(3  ({{\bf{\hat{\Delta}}}_{ji}\cdot{\bf{\hat{r}}}_i^{b}})^2 - 1 \Big)-\frac{{\cal G} }{2\Delta_{ji}^3} \mathcal{C}_i \biggl( {\mathcal E}^{z}_i - \frac{1}{2} {\mathcal E}^{\rho}_i 
\biggr),
\end{split}
\label{eq13}
\end{eqnarray}

%${\bf{\hat{\Delta}}}_{ji}\cdot{\bf{\hat{r}}}_i^{(b)}} = \cos{( \varphi_{ji} - (\varphi^{(eq)}_i + \delta_i))}$.
where $A_i,B_i,C_i$ are the principal moments of inertia of $m_i$ which can be related to the ellipsoidal flattenings (see \cite{Folonier2015}, Appendix A) as:
\begin{equation}
(B_i-A_i) \simeq \mathcal{C}_i {\mathcal E}^{\rho}_i \hspace*{0.5cm} ; \hspace*{0.5cm} 
(C_i-B_i) \simeq \mathcal{C}_i \biggl( {\mathcal E}^{z}_i - \frac{1}{2} {\mathcal E}^{\rho}_i 
\biggr) ,
\label{eq15}
\end{equation}
 where $\mathcal{C}_i= (2/5) m_i \mathcal{R}_i^2$ is the principal moment of inertia of a homogeneous  spherical body of mass $m_i$ and radius $\mathcal{R}_i$.
 
The tidal force applied on $m_j$ due to the deformation of $m_i$ can be simply calculated as:
\begin{eqnarray}
\label{eq:fuerza}
{\bf{F}}_{ji} &=& -m_j \nabla_{{\bf \Delta}_{ji}} U_{ji} \nonumber \\
&=& \frac{3{\cal G}m_j \mathcal{C}_i}{2\Delta_{ji}^5}{\mathcal E}^{\rho}_i\sin{(2(\varphi^{eq}_i+\delta_i)-2\varphi_{ji})}\ (\hat{\bf{k}}\times{\bf{\Delta}}_{ji}) \nonumber \\
&-&\frac{3{\cal G}m_j \mathcal{C}_i}{2\Delta_{ji}^5} \Big(\frac{3}{2}{\mathcal E}^{\rho}_i\cos{(2(\varphi^{eq}_i+\delta_i)-2\varphi_{ji})}+{\mathcal E}^{z}_i\Big){\bf{\Delta}}_{ji},
\end{eqnarray}
where we have decomposed $\hat {\bf{r}}_i^{b}$ in terms of the radial unit vector $\hat{\bf{\Delta}}_{ji}$ and the azimutal unit vector $(\hat{\bf{k}} \times \hat{\bf{\Delta}}_{ji})$ ( 
$\hat{\bf{k}}$ is the unit vector paralell to the spin vectors)

The torque induced on $m_j$ due to the deformation of $m_i$ can be simply calculated as 
\begin{equation}
\begin{split}
{\bf{T}}_{ji} &= {\bf{\Delta}}_{ji} \times {\bf{F}}_{ji} \\
              &= \frac{3{\cal G}m_j \mathcal{C}_i}{2\Delta_{ji}^3}{\mathcal E}^{\rho}_i\sin{(2(\varphi^{eq}_i+\delta_i)-2\varphi_{ji})}\ \hat{\bf{k}}
\end{split}
\label{eq:tji}
\end{equation}

Now, we assume that the reaction torque due to the deformation on $m_i$ will be the only responsable in changing its spin. This is a natural assumption that satisfies that, in the limit when $\mathcal{R}_i \to 0$, the variation in the rotation speed of $m_i$ is also cancelled  (see \cite{Zoppetti2019}). Thus, the rotational evolution of $m_i$ is given by
\begin{eqnarray}
C_i \dot{{\bf{\Omega}}}_{i} + \dot{C}_i {{\bf{\Omega}}}_{i} &=& - \Big( {{\bf{T}}}_{ji} + {{\bf{T}}}_{ki}  \Big) \\
&=&-\frac{3{\cal G} \mathcal{C}_i{\mathcal E}^{\rho}_i}{2}\bigg[\frac{m_j}{\Delta_{ji}^3}\sin{(2(\varphi^{eq}_i+\delta_i)-2\varphi_{ji})} \\
&+&\frac{m_k}{\Delta_{ji}^3}\sin{(2(\varphi^{eq}_i+\delta_i)-2\varphi_{ki})}\ \bigg]  \hat{\bf{k}}
\label{eq:torque}
\end{eqnarray}

If we neglect in the variation of the angular momentum of spin (Equation \ref{eq:torque}) the term corresponding to the variation of the polar moment of inertia, using Equations (\ref{formaeq}) and after some algebra, the rotational evolution of the body  $m_i$ will be governed by 
\begin{equation}
\label{eq:spins}
\dot{\Omega}_{i} &= 
-\frac{2{\cal G} m_i}{5 \mathcal{R}_i^3} \epsilon_i^{(\rho)} Y_i \\
\end{equation}

The set of differential equations formed by Equations
(\ref{eq:forma}) and (\ref{eq:spins}) described the dynamical evolution of each of the three bodies of the system on short timescales and will be target of this work. The orbital evolution on long timescales, descripted by the Newton third law with expression for the forces given in Equation \ref{eq:fuerza} will be addressed in a forthcoming work.  



\section{An analytical solution for the rotational stationary state}

It is possible to identify that there mainly two different timescales involved in the problem. Over short timescales, it is expected that the shape, orientation and rotation acquire stationary solution and oscillate around those values. On the other hand, only periodic oscillations are expected in the orbital elements with the exception of the fast angles over this short timescales. For this reason, in this work we take advantage of this adiabatic nature of the problem and solve the set of differential equation associated with the variation of the shape of each body, its orientation and its rotation (Equations (\ref{eq:forma}) and (\ref{eq:spins}), assuming fixed values for all the orbital elements with the exception of the true anomalies. \\
We now search for an analytical approximation, for each body $m_i$, to the flattenings and orientation represented by $(X_i,Y_i,{\mathcal E}^{z}_i)$ and also to the rotation $\Omega_i$ in the quasi-synchronous atractor. To do this, we first adopt a Jacobi reference frame for the coordinates and velocities, where the state vector of the secondary $m_1$ is defined as $m_0$-centric, while the state vector of $m_2$ is measured with respect to the barycenter of $m_0$ and $m_1$. Due to the symmetry of the Jacobian system, we will consider the solution for the central bodies and, separately, the solution for the external mass. 

\subsection{The central bodies}
\label{centralb}
Then, we assume the particular solution for the two central bodies given by
\begin{eqnarray}
X_i = \langle X_i \rangle + ... \\
Y_i = \langle Y_i \rangle + ... \\
\mathcal{E}^z_i = \langle \mathcal{E}^z_i \rangle + ... \\
\Omega_i = \langle\Omega_i\rangle + ..., 
\end{eqnarray}
for $i=0,1$. 
\begin{eqnarray}
\langle \Omega_0 \rangle &=& n_1 + 6\frac{\gamma_0^2 n_1}{\gamma_0^2+n_1^2}  e_1^2 \nonumber \\ 
 &-& \bigg[ \frac{1}{4} \frac{m_2}{m_0+m_1}\frac{\gamma_0^2n_1}{\gamma_0^2+n_1^2}  e_1 e_2 \cos(\Delta \varpi) \bigg] \alpha^4 \nonumber \\
&-& \bigg[ \frac{15}{4} \frac{m_1 m_2}{{(m_0+m_1)}^2}\frac{\gamma_0^2n_1}{\gamma_0^2+n_1^2}  e_1^2
\bigg] \alpha^5 \nonumber \\
&-&  \bigg[ (\frac{m_2}{m_1})}^2 \frac{\gamma_0^2}{\gamma_0^2+{(2n_1-2n_2)}^2} (2n_1-2n_2) \nonumber \\
+ \frac{25}{4} \frac{m_2 m_1^2}{{m0+m1}^3}} \frac{\gamma_0^2}{\gamma_0^2+{n_1}^2} n_1 e_1 e_2 \cos(\Delta \varpi) \nonumber \\ 
+\frac{\gamma_0^2}{\gamma_0^2+{(2n_1-3n_2)}^2} \bigg[(25n_1-37n_2)- \frac{n_2(2n_1-n_2)(2n_1-2n_2)}{\gamma_0^2+{(2n_1-n_2)}^2}    \bigg]  e_2^2 \nonumber \\
+ FALTA e_1^2 \bigg]] \alpha^6 \nonumber  %\langle \Omega_1 \rangle &=& n_1 + 6\frac{\gamma_1^2 n_1}{\gamma_1^2+n_1^2}  e_1^2 \nonumber \\ 
% &+& \bigg[ \frac{1}{4} \frac{m_2}{m_0+m_1}\frac{\gamma_1^2n_1}{\gamma_1^2+n_1^2}  e_1 e_2 \cos(\Delta \varpi) \bigg] \alpha^4 \nonumber 
\end{eqnarray}


\subsection{The external body}
Similarly to the previous Section (\ref{centralb}), we assume the following particular solution for the two central bodies given by
\begin{eqnarray}
X_2 = \langle X_2 \rangle + ... \\
Y_2 = \langle Y_2 \rangle + ... \\
\mathcal{E}^z_2 = \langle \mathcal{E}^z_2 \rangle + ... \\
\Omega_2 = \langle\Omega_2\rangle + ..., 
\end{eqnarray}

We choose to express the stationary solution for the shape and orientation explicitly in terms of the flattenings ( $\mathcal{E}^\rho_i$ and $\mathcal{E}^z_i$) and orientation lag $\delta_i$ 
\begin{eqnarray} 
\langle \delta_2 \rangle &=&  6\frac{\gamma_2 n_2}{\gamma_2^2+n_2^2}  e_2^2 \nonumber \\ 
&+& \bigg[5 M_2 \frac{\gamma_2 n_2}{\gamma_2^2+n_2^2} e_2^2 \bigg] \alpha^2  \\
&-& \bigg[ \frac{19}{2} M_2^2  \frac{\gamma_2 (2n_1-2n_2)}{\gamma_2^2+{(2 n_1-2n_2)}^2} \bigg] \alpha^4 \\ \frac{\langle {\mathcal E}^\rho_2 \rangle}{\overline{\epsilon}^\rho_2} &=&  1 + \bigg(\frac{3}{2} - 8 \frac{n_2^2}{\gamma_2^2+n_2^2} \bigg) e_2^2 \nonumber \\ 
&+& \bigg[ \frac{5}{4}+\frac{15}{8}e_1^2 + \bigg( \frac{25}{4} - 10 \frac{n_2^2}{\gamma_2^2+n_2^2} \bigg) e_2^2 \bigg]  M_2 \alpha^2  \\
&+& \bigg[ \frac{105}{64} M_4 + 4    \frac{\gamma_2^2 - {(2n_1-2n_2)}^2}{\gamma_2^2 + {(2n_1-2n_2)}^2} M_2^2 \bigg] \alpha^4 \nonumber %- \frac{M_2^2}{2} 
\end{eqnarray}

\begin{eqnarray}
 \langle \Omega_2 \rangle &=& n_2 + 6\frac{\gamma_2^2 n_2}{\gamma_2^2+n_2^2}  e_2^2 
+ \bigg[5 M_2 \frac{\gamma_2^2n_2}{\gamma_2^2+n_2^2} e_2^2 \bigg] \alpha^2 \\
%&-& \bigg[ \frac{325}{16} M_3\frac{\gamma_2^2n_2}{\gamma_2^2+n_2^2}  e_1 e_2 \cos(\Delta \varpi) \bigg] \alpha^3 \nonumber \\
&-& \bigg[ \frac{19}{2} M_2^2  \frac{\gamma_2^2(2n_1-2n_2)}{\gamma_2^2+{(2 n_1-2n_2)}^2} \bigg] \alpha^4 %- \frac{M_2^2}{2} 
\end{eqnarray}







\section{La sol de gabriel}
If we also consider that, in the variation of the angular momentum of spin (Equation \ref{eq:varmas}), the term corresponding to the variation of the polar moment of inertia is negligible, the set of differential equations to be solved is reduced to
\begin{eqnarray}
\label{eq:sist}
\begin{split}
\dot{X_i} &= -\gamma_i X_i -2 Y_i (\Omega_i-\dot{\varphi_i}^{(eq)})+\gamma_i \epsilon_i^{(\rho)} \\
\dot{Y_i} &= -\gamma_i Y_i +2 X_i (\Omega_i-\dot{\varphi_i}^{(eq)}) \\
\dot{\Omega}_{i} &= 
-\frac{2{\cal G} m_i}{5 \mathcal{R}_i^3} \epsilon_i^{(\rho)} Y_i \\
\dot{{\mathcal E}_i}^{(z)} &=-\gamma_i {{\mathcal E}_i}^{(z)} + \gamma_i {\epsilon_i}^{(z)}
\end{split}
\end{eqnarray}

We first notice that the evolution equation associated to the polar flattening (last Equation in system (\ref{eq:sist}) is decoupled from the rest and can be solved separately, once the solution for $\Omega_i$ is known.\\
Secondly, as discussed in \cite{Gomes2019}, the typical timescales of spins evolution is much slower than those associated to the shape and orientation. For this reason, although it is not a self-consistent way, a very accurate solution is obtained when we assume that $\Omega_i \sim const.$ to solve the shape and orientation evolution of each body, and then use the torque expression to obtain the spin evolution.\\
Following \cite{Gomes2019}, the solution for the regular variables can be obtained

\begin{eqnarray}
\label{eq:xy}
 X_i +i Y_i = \gamma_i e^{-\gamma_it+2i(\Omega_it-\varphi_i^{(eq)})}\int \epsilon_i^{(\rho)} e^{\gamma_it-2i(\Omega_it-\varphi_i^{(eq)})}\ dt
\end{eqnarray}

To analytically solve the integral in Equation (\ref{eq:xy}) we need to use eliptical expansion for the term

\begin{equation}
 \epsilon_i^{(\rho)} e^{i2\phi_i^{(eq)}} = \sum_{\bf{p}\in \mathbf{Z}^4} \mathcal{A}^i_{\bf{p}} e^{i\phi^i_{\bf{p}}}
 \label{expantion_gral}
\end{equation}
where $\phi^i_{\bf{p}}=p_1M_1+p_2M_2+p_3\varpi_1+p_4\varpi_2$ and $\mathcal{A}^i_{\bf{p}}$ are real coefficients. After some algebra it is possible to find that

\begin{eqnarray}
 X_i = \frac{\gamma_i}{\epsilon_i^{(\rho)}} \sum_{\bf{p,p'}\in \mathbf{Z}^4} \mathcal{A}^i_{\bf{p}}\mathcal{A}^i_{\bf{p'}} \frac{\gamma_i \sin(\phi^i_{\bf{p}}+\phi^i_{\bf{p'}})+(2\Omega_i-\dot{\phi^i}_{\bf{p}})\cos(\phi^i_{\bf{p}}+\phi^i_{\bf{p'}})}{\gamma_i^2+{(2\Omega_i-\dot{\phi^i}_{\bf{p}})}^2} \\ 
 Y_i = \frac{\gamma_i}{\epsilon_i^{(\rho)}} \sum_{\bf{p,p'}\in \mathbf{Z}^4} \mathcal{A}^i_{\bf{p}}\mathcal{A}^i_{\bf{p'}} \frac{\gamma_i \sin(\phi^i_{\bf{p}}-\phi^i_{\bf{p'}})+(2\Omega_i-\dot{\phi^i}_{\bf{p}})\cos(\phi^i_{\bf{p}}-\phi^i_{\bf{p'}})}{\gamma_i^2+{(2\Omega_i-\dot{\phi^i}_{\bf{p}})}^2}\\
 \dot{\Omega}_i = -\frac{2\mathcal{G}m_i}{5\mathcal{R}_i^3}\gamma_i\sum_{{\bf{p}},{\bf{p}'}}\mathcal{A}^i_{\bf{p}}\mathcal{A}^i_{\bf{p}'}\frac{\gamma_i \sin(\phi^i_{\bf{p}}-\phi^i_{\bf{p'}})+(2\Omega_i-\dot{\phi^i}_{\bf{p}})\cos(\phi^i_{\bf{p}}-\phi^i_{\bf{p'}})}{\gamma_i^2+{(2\Omega_i-\dot{\phi^i}_{\bf{p}})}^2}
 \label{expantion_gral}
\end{eqnarray}



\section{Conclusions}
La tesis de zoppetti, defendida en mayo de 2020 y cuya version final aun no ha sido publicada esta mal.

\section*{Appendix A: High order terms}
\begin{eqnarray}
 \langle\delta\Omega_2\rangle&=&-\frac{5M_2 (n_1-n_2)\gamma_2^2\alpha^6 }{32\left(\gamma_2^2+(n_1-n_2)^2\right)
 \left(\gamma_2^2+4(n_1-n_2)^2\right) \left(\gamma_2^2+9(n_1-n_2)^2\right)}\nonumber\\
&&\times \Big((121\gamma_2^4+805\gamma_2^2(n_1-n_2)^2+744(n_1-n_2)^4)5M_4\\
&&\qquad -(729\gamma_2^4+5265\gamma_2^2(n_1-n_2)^2 +4836(n_1-n_2)^4) M_2^2\nonumber \Big)
\end{eqnarray}

\begin{equation}
 \langle\delta\delta_2\rangle = \frac{\langle\delta\Omega_2\rangle}{\gamma_2}
\end{equation}

\begin{eqnarray}
\frac{\langle\delta\mathcal{E}^\rho_2\rangle}{\overline{\epsilon}^\rho_2}&=&\frac{5M_2\alpha^6}{256\left(\gamma_2^2+(n_1-n_2)^2\right) \left(\gamma_2^2+4 (n_1-n_2)^2\right) \left(\gamma_2^2+9 (n_1-n_2)^2\right)}\nonumber\\
&&\times\Big(\gamma_2^6 \mathcal{F}_1 +70 \gamma_2^4(n_1-n_2)^2 \mathcal{F}_2\\
&&\qquad+\gamma_2^2(n_1-n_2)^4 \mathcal{F}_3+378(n_1-n_2)^6\mathcal{F}_4 \Big)\nonumber
\end{eqnarray}

\begin{equation}
 \frac{\langle\delta\mathcal{Z}^z_2\rangle}{\overline{\epsilon}^\rho_2}=\frac{1225 M_2\mathcal{F}_4\alpha^6}{512}
\end{equation}

\begin{equation}
\frac{\langle\delta\mathcal{Q}^z_2\rangle}{\overline{\epsilon}^M_2} = \frac{2\langle\delta\Omega_2\rangle}{n_2}\end{equation}

\begin{eqnarray}
 \mathcal{F}_1 &=& \frac{105 m_0^4+671 m_0^3 m_1-1447 m_0^2 m_1^2+671 m_0 m_1^3+105 m_1^4}{(m_0+m_1)^4} \nonumber\\
 \mathcal{F}_2 &=& \frac{21 m_0^4+55 m_0^3 m_1-131 m_0^2 m_1^2+55 m_0 m_1^3+21 m_1^4}{(m_0+m_1)^4} \nonumber\\
 \mathcal{F}_3 &=& \frac{5145 m_0^4-121 m_0^3 m_1-4903 m_0^2 m_1^2-121 m_0 m_1^3+5145 m_1^4}{(m_0+m_1)^4} \nonumber\\
 \mathcal{F}_4 &=& \frac{m_0^4-m_0^3 m_1+m_0^2 m_1^2-m_0 m_1^3+m_1^4}{(m_0+m_1)^4}.
\end{eqnarray}

\section*{metiendo mano}

\begin{eqnarray}
 \langle\delta\Omega_2\rangle&=&-\frac{5M_2}{32}   \frac{(n_1-n_2)\gamma_2^2\alpha^6 }{\left(\gamma_2^2+(n_1-n_2)^2\right)
 \left(\gamma_2^2+4(n_1-n_2)^2\right) \left(\gamma_2^2+9(n_1-n_2)^2\right)}\nonumber\\
&&\times \Big[ 5M_4 \Big(121\gamma_2^4+805\gamma_2^2(n_1-n_2)^2+744(n_1-n_2)^4 \Big)\\
&&\qquad -3M_2^2 \Big(243\gamma_2^4+1755\gamma_2^2(n_1-n_2)^2 +1612(n_1-n_2)^4 \Big) \nonumber \Big]
\end{eqnarray}

\begin{equation}
 \langle\delta\delta_2\rangle = \frac{\langle\delta\Omega_2\rangle}{\gamma_2}
\end{equation}

\begin{eqnarray}
\frac{\langle\delta\mathcal{E}^\rho_2\rangle}{\overline{\epsilon}^\rho_2}&=&\frac{5M_2}{256}\frac{\alpha^6}{\left(\gamma_2^2+(n_1-n_2)^2\right) \left(\gamma_2^2+4 (n_1-n_2)^2\right) \left(\gamma_2^2+9 (n_1-n_2)^2\right)}\nonumber\\
&&\times \Big[(105\mathcal{F}_1+776\mathcal{F}_2)\gamma_2^6  +70 (21\mathcal{F}_1+76\mathcal{F}_2)\gamma_2^4(n_1-n_2)^2\\
&&\qquad+(5145\mathcal{F}_1+5024\mathcal{F}_2)\gamma_2^2(n_1-n_2)^4+378\mathcal{F}_1 (n_1-n_2)^6 \Big]\nonumber
\end{eqnarray}

\begin{equation}
 \frac{\langle\delta\mathcal{Z}^z_2\rangle}{\overline{\epsilon}^\rho_2}=\frac{1225}{512}\frac{\beta (1+\beta^5)}{(1+\beta^7)}\alpha^6
\end{equation}

\begin{equation}
\frac{\langle\delta\mathcal{Q}^z_2\rangle}{\overline{\epsilon}^M_2} = \frac{2\langle\delta\Omega_2\rangle}{n_2}\end{equation}

\begin{eqnarray}
\mathcal{F}_1 &=& \frac{1+\beta^5}{(1+\beta)^5}\nonumber\\
\mathcal{F}_2 &=& \frac{\beta (1-\beta)^2}{(1+\beta)^4}.
\end{eqnarray}



\begin{acknowledgements}
      Part of this work was supported by the German
      \emph{Deut\-sche For\-schungs\-ge\-mein\-schaft, DFG\/} project
      number Ts~17/2--1.
\end{acknowledgements}

% WARNING
%-------------------------------------------------------------------
% Please note that we have included the references to the file aa.dem in
% order to compile it, but we ask you to:
%
% - use BibTeX with the regular commands:
%   \bibliographystyle{aa} % style aa.bst
%   \bibliography{Yourfile} % your references Yourfile.bib
%
% - join the .bib files when you upload your source files
%-------------------------------------------------------------------

\begin{thebibliography}{}

\bibitem[Ferraz-Mello(2013)]{FerrazMello2013} Ferraz-Mello, S.\ 2013, Celestial Mechanics and Dynamical Astronomy, 116, 109

\bibitem[Folonier et al.(2015)]{Folonier2015}
Folonier, H.~A., Ferraz-Mello, S., \& Kholshevnikov, K.~V.\ 2015, Celestial Mechanics and Dynamical Astronomy, 122, 183.

\bibitem[Folonier et al.(2018)]{Folonier2018} 
Folonier, H.~A., Ferraz-Mello, S., \& Andrade-Ines, E.\ 2018, Celestial Mechanics and Dynamical Astronomy, 130, 78.

\bibitem[Gomes et al.(2019)]{Gomes2019}
Gomes, G.~O., Folonier, H.~A., \& Ferraz-Mello, S.\ 2019, Celestial Mechanics and Dynamical Astronomy, 131, 56

\bibitem[Murray \& Dermott(1999)]{Murray1999}
Murray, C.~D., \& Dermott, S.~F.\ 1999, Solar system dynamics by C.D. Murray and S.F. McDermott. (Cambridge


\bibitem[Tisserand (1891)]{Tisserand1891} Tisserand, Félix. Traité de mécanique céleste. Gauthier-Villars, 1891.

\bibitem[Zoppetti et al.(2019)]{Zoppetti2019} 
Zoppetti, F.~A., Beaug{\'e}, C., Leiva, A.~M., et al.\ 2019, \aap, 627, A109

\end{thebibliography}

\end{document}

